Nucleon structure functions with domain wall fermions

We present a quenched lattice QCD calculation of the first few moments of the polarized and un-polarized structure functions of the nucleon. Our calculations are done using domain wall fermions and the DBW2 gauge action with inverse lattice spacing ~1.3GeV, physical volume approximatelly (2.4 fm)^3, and light quark masses down to about 1/4 the strange quark mass. Values of the individual moments are found to be significantly larger than experiment, as in past lattice calculations, but interestingly the chiral symmetry of domain wall fermions allows for a precise determination of the ratio of the flavor non-singlet momentum fraction to the helicity distribution, which is in very good agreement with experiment. We discuss the implications of this result. Next, we show that the chiral symmetry of domain wall fermions is useful in eliminating mixing of power divergent lower dimensional operators with twist-3 operators. Finally, we find the isovector tensor charge at renormalization scale 2 GeV in the MS bar scheme to be 1.192(30), where the error is the statistical error only.

==> text_sections/LatticeRenorm.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%  Section %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  \section{Renormalization Constants}
%  \label{sec:LatticeRenorm}
%  File:  LatticeRenorm.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ifnum\theOutline=1
\begin{outline}
\item NPR simulation details
\item Plateaus
\item fits
\item Z factors in MSbar at 2GeV
\end{outline}
\fi


